Robust Quantization: One Model to Rule Them All

Neural network quantization methods often involve simulating the quantization process during training, making the trained model highly dependent on the target bit-width and precise way quantization is performed. Robust quantization offers an alternative approach with improved tolerance to different classes of data-types and quantization policies. It opens up new exciting applications where the quantization process is not static and can vary to meet different circumstances and implementations. To address this issue, we propose a method that provides intrinsic robustness to the model against a broad range of quantization processes. Our method is motivated by theoretical arguments and enables us to store a single generic model capable of operating at various bit-widths and quantization policies. We validate our method's effectiveness on different ImageNet models.

==> sections/02_related_draft.tex <==
\section{Related work}
\RB{text here is too long and overly written. It gives unimportant details. Perhaps remove the PTQ and QAT and leave only the last paragraph related to robustness. We need to keep this section clear and focused. }
\label{related_work}
% \BCH{There is some problem with citation }

Quantization techniques may be divided into post-training quantization (PTQ) and quantization-aware training (QAT).
The former, as the name implies, does not comprise training of the model parameters.
Instead, PTQ techniques mainly involve clipping of the pretrained model distributions of the activations and/or weights followed by their linear quantization.
The lack of training is usually reflected in lesser performance compared to QAT; however, QAT requires resources for training that may not be available, such as the training dataset, energy, or time.

\textbf{Post-training quantization.}
PTQ methods vary mainly in the way the clipping is performed.
\citep{banner2018post} and \citep{choukroun2019low} find optimal clipping values in terms of the mean-squared-error (MSE), \citep{migacz20178} pick clipping values that minimize the Kullback-Leibler (KL) divergence, and \citep{gong2018highly} use the $L_\infty$ norm.
Clipping may be also accompanied by minor distribution tweaking.
\citep{zhao2019improving} address the importance of clipping outlier values and propose outlier channel splitting; 
% \citep{nayak2019bit} perform hierarchical clustering of classes to help the quantized model differentiate between overlapping class distributions; and \citep{finkelstein2019fighting} correct the mean activation value shift in the quantized model with bias.
\citep{finkelstein2019fighting} correct the mean activation value shift in the quantized model with bias.
Clipping may also be considered in channel granularity \citep{lee2018quantization}, and its value may be obtained according to the global network loss function \citep{nahshan2019loss}.



\textbf{Quantization-aware training.}
QAT methods optimize model parameters for quantization with gradient descent and backpropagation.
Quantization step size (\citep{choi2018pact,baskin2018nice,esser2019learned,zhang2018lq,Zhou2016DoReFaNetTL}), for example, may also be defined as a learnable parameter.
% , thereby optimally adjusted during the training procedure.
Since QAT passes model activations and/or weights through ``quantization layers'', and since quantization operations are not differentiable, it is common to employ a straight-through estimator \citep{steBengioLC13}.
Differentiable models of the quantizer have been shown to improve the performance of QAT (\citep{yang2019quantization,gong2019differentiable,elthakeb2019sinreq}).


\textbf{Robustness and distribution reshaping.}
\RB{Referecnes at the beginning of a sentence should use citet{} and not citep{}}\citet{alizadeh2020robustquantization} seeks to improve the robustness of the model as well. While \citep{alizadeh2020robustquantization} demonstrates only bit-width robustness, we also show robustness to quantization step size. In addition, \citep{alizadeh2020robustquantization} focuses on such improvement when using PTQ methods. Our work shows an improvement for both PTQ and QAT.
Last, \citep{alizadeh2020robustquantization}'s solution significantly extends the model generation time while our solution does not have a significant impact on this period of time. \MR{what about the results themselves?}
% Another related work by \citep{Yu2019GDRQGD} describes a uniformization of the model distributions, targeting, however, a very different goal. While \citep{Yu2019GDRQGD} proposed a QAT scheme, we propose a complementary method to PTQ and QAT that produces models robust to different quantization techniques. In addition, we prove that uniformly-distributed tensors are indeed more resilient to noise.
Another related work by \citep{Yu2019GDRQGD} describes a uniformization of the model distributions by imposing clipping during training. \citep{Yu2019GDRQGD} targets, however, a very different goal. While \citep{Yu2019GDRQGD} proposed a QAT scheme, we propose a complementary method to PTQ and QAT that produces models robust to different quantization techniques. In addition, we prove that uniformly-distributed tensors are indeed more resilient to noise.


==> sections/03_method.tex <==
\section {Model and problem formulation}
\label{sec:model_problem_formulation}

Given a uniform $M$-bit quantizer with quantization step size $\Delta$ that maps a continuous value $x\in \mathbb{R}$ into a discrete representation $Q_{\Delta}(x)=i\cdot \Delta$ with $ i\in \{0,1,..., 2^M -1\}$.  The index $i$ is expressed as follows: \MR{write it clearer}
\begin{equation}
    i=\left \lfloor{\dfrac{x}{\Delta}}\right \rfloor \,.
\end{equation}


Given a random variable $X$ taken from a distribution $f$ and a quantizer $Q_{\Delta}(X)$, we consider the expected mean-squared-error (MSE) as a local distortion measure we would like to minimize, that is,
\begin{equation}
\text{MSE}(X,\Delta) = \mathbb{E}\left[\left(X- Q_{\Delta}(X)\right)^2\right] \,.
\end{equation}

Assuming an optimal quantization step $\tilde{\Delta}$ and optimal quantizer $Q_{\tilde{\Delta}}(X)$ for a given distribution $X$, we quantify the quantization sensitivity $\Gamma(X,\epsilon)$ as the increase in $\text{MSE}(X,\Delta)$ following a small changes in the optimal quantization step size $\tilde{\Delta}(X)$. Specifically, for a given $\epsilon>0$ and a quantization step size $\Delta$ around $\tilde{\Delta}$ (i.e., $|\Delta - \tilde{\Delta}|= \epsilon$) we measure the following difference: 
\begin{equation}
\label{robustness_definition}
    \Gamma(X,\epsilon) = \left|\text{MSE}(X,\Delta) - \text{MSE}(X,\tilde{\Delta})\right| \,.
\end{equation}
The following Lemma will be useful to estimate the quantization sensitivity $\Gamma(X,\epsilon)$  for various density distributions. 

\begin{lemma}
\label{Lemma1}
Assuming a second order Taylor approximation, the quantization sensitivity $\Gamma(X,\epsilon)$ satisfies the following equation:
\begin{equation}
\Gamma(X,\epsilon) =  \left | \frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \right| \,.
\end{equation}
\end{lemma}


\textbf{Proof:} \MR{move to supplementary material} Let $\Delta'$ be a quantization step with similar size to $\tilde{\Delta}$ so that $|\Delta' - \tilde{\Delta}|=\epsilon$.
Using a second order Taylor expansion, we approximate $\text{MSE}(X,\Delta')$ around $\tilde{\Delta}$ as follows:
% \begin{equation}
% \begin{split}
% \text{MSE}(X,\Delta') &= \text{MSE}(X,\tilde{\Delta}) \\
% &+ \frac{\partial \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial \Delta} (\Delta'-\tilde{\Delta}) \\
% &+ \frac{1}{2}\cdot\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} (\Delta'-\tilde{\Delta})^2 \\
% &+O(\Delta'-\tilde{\Delta})^3 \,.
% \end{split}
% \label{taylor}
% \end{equation}

\begin{equation}
\begin{split}
\text{MSE}(X,\Delta') &= 
\text{MSE}(X,\tilde{\Delta}) 
+ \frac{\partial \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial \Delta} (\Delta'-\tilde{\Delta}) \\
&+ \frac{1}{2}\cdot\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} (\Delta'-\tilde{\Delta})^2 
+O(\Delta'-\tilde{\Delta})^3 \,.
\end{split}
\label{taylor}
\end{equation}


Since $\tilde{\Delta}$ is the optimal quantization step for $\text{MSE}(X,\Delta)$, we have that $\frac{\partial \text{mse}(X, \Delta= \tilde{\Delta})}{\partial \Delta}=0$. In addition, by ignoring order terms higher than two, we can re-write Equation~(\ref{taylor}) as follows:
% \begin{equation}
% \label{eq1}
% \begin{split}
%  \text{MSE}(X,\Delta') &- \text{MSE}(X,\tilde{\Delta})=\\
% &=\frac{1}{2}\cdot\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} (\Delta'-\tilde{\Delta})^2 \\ 
% &=\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \,.
% \end{split}
% \end{equation} 

\begin{equation}
\label{eq1}
 \text{MSE}(X,\Delta') - \text{MSE}(X,\tilde{\Delta})=\\
\frac{1}{2}\cdot\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} (\Delta'-\tilde{\Delta})^2 \\ 
=\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \,.
\end{equation} 


Equation~(\ref{eq1}) holds also with absolute values:
% \begin{equation}
% \label{eq2}
% \begin{split}
% \Gamma(X,\epsilon) &= \left|\text{MSE}(X,\Delta') - \text{MSE}(X,\tilde{\Delta})\right|\\
% &=\left|\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2}\right| \,.
% \end{split}
% \end{equation} $\blacksquare$

\begin{equation}
\label{eq2}
\Gamma(X,\epsilon) = \left|\text{MSE}(X,\Delta') - \text{MSE}(X,\tilde{\Delta})\right|\\
=\left|\frac{\partial^2 \text{MSE}(X, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2}\right| \,.
\end{equation} $\blacksquare$


In the next subsection, we use Lemma~\ref{Lemma1} to compare the quantization sensitivity of the Normal distribution with and Uniform distribution.  

\subsection{Robustness of tensor distributions}
In this section, we consider different tensor distributions and their robustness to quantization. Specifically, we show that for a tensor $X$ with a uniform distribution $Q(X)$ the variations in the region around $Q(X)$ are smaller compared with other typical distributions of weights and activations. This is captured through the following theorem.
\begin{lemma}
Let $X_U$ be a continuous random variable that is uniformly distributed in the interval $[-a,a]$. Assume that $Q_{\Delta}(X_U)$ is a uniform $M$-bit quantizer with a quantization step $\Delta$. Then, the expected MSE is given as follows:
\begin{equation*}
    \text{\text{MSE}}(X_U,\Delta)  = \frac{(a-2^{M-1}\Delta)^3}{3a} + \frac{2^M\cdot\Delta^3}{24a} \,.
\end{equation*}
\label{lemma_uniform_dist}
\end{lemma}
\textbf{Proof:} Given a finite quantization step size $\Delta$ and a finite range of quantization levels $2^M$, the quanitzer truncates input values larger than $2^{M-1}\Delta$ and smaller than $-2^{M-1}\Delta$.  Hence, denoting by $\tau$ this threshold (i.e., $\tau \triangleq 2^{M-1}\Delta$), the quantizer can be modeled as follows:
\begin{equation}
    Q_{\Delta}(x) = \left\{\begin{alignedat}{2}
        & \tau & x  &> \tau \\
        & \Delta\cdot \left\lfloor \frac { x } { \Delta } \right\rceil \qquad & |x| &\leq \tau \\
        & -\tau & x  &< -\tau \,.
    \end{alignedat}\right. 
\end{equation}

Therefore, by the law of total expectation, we know that 
\begin{equation}
    \begin{array} { l } { \mathbb{E}\left[\left(x- Q_{\Delta}(x)\right)^2\right]=}\\
    {  \mathbb{E} \left[ \left( x - \tau \right) ^ { 2 } \mid x> \tau\right] \cdot P \left[ x > \tau \right] +} 
    \\
     { \mathbb{E} \left[ \left( x - \Delta\cdot \left\lfloor \frac { x } { \Delta } \right\rceil \right) ^ { 2 } \mid |x|\leq \tau  \right ] \cdot P \left[ |x| \leq \tau \right] +} \\ 
     {\mathbb{E} \left[ \left( x + \tau \right) ^ { 2 } \mid x < -\tau \right] \cdot P \left[ x  < -\tau \right] \,. }
    \end{array} 
    \label{total_expectation}
\end{equation}

% \begin{equation}
%     \begin{array} { l } { \mathbb{E}\left[\left(x- Q_{\Delta}(x)\right)^2\right]=}
%     {  \mathbb{E} \left[ \left( x - \tau \right) ^ { 2 } \mid x> \tau\right] \cdot P \left[ x > \tau \right] +} 
%     \\
%      { \mathbb{E} \left[ \left( x - \Delta\cdot \left\lfloor \frac { x } { \Delta } \right\rceil \right) ^ { 2 } \mid |x|\leq \tau  \right ] \cdot P \left[ |x| \leq \tau \right] +} 
%      {\mathbb{E} \left[ \left( x + \tau \right) ^ { 2 } \mid x < -\tau \right] \cdot P \left[ x  < -\tau \right] \,. }
%     \end{array} 
%     \label{total_expectation}
% \end{equation}

We now turn to evaluate the contribution of each term in Equation~(\ref{total_expectation}). We begin with the case of $x>\tau$, for which the probability density is uniform in the range $[\tau,a]$ and zero for $x>a$. Hence, the conditional expectation is given as follows: 
% \begin{equation}
% \begin{split} \mathbb{E} \left[ \left( x - \tau \right) ^ { 2 } \mid x> \tau\right] &= \int _ { \tau } ^ { a } ( x - \tau ) ^ { 2 } \cdot d x \\
% &= \frac{1}{3}\cdot ( a - \tau ) ^ { 3 } \,.
% \end{split}
% \end{equation}
\begin{equation}
\mathbb{E} \left[ \left( x - \tau \right) ^ { 2 } \mid x> \tau\right] = \int _ { \tau } ^ { a } ( x - \tau ) ^ { 2 } \cdot d x \\
= \frac{1}{3}\cdot ( a - \tau ) ^ { 3 } \,.
\end{equation}
In addition, since $x$ is uniformly distributed in the range $[-a,a]$, a random sampling from the interval $[\tau, a]$ happens with a probability 
\begin{equation}
    P \left[ x > \tau \right] = \frac{a-\tau}{2a} \,.
\end{equation}
Therefore, the first term in Equation~(\ref{total_expectation}) is stated as follows:
\begin{equation}
\mathbb{E} \left[ \left( x - \tau \right) ^ { 2 } \mid x> \tau\right] \cdot    P \left[ x > \tau \right] = \frac{(a-\tau)^3}{6a} \,.
\label{tail}
\end{equation}
Since $x$ is symmetrical around zero, the first and last terms in Equation~(\ref{total_expectation}) are equal and their sum can be evaluated by multiplying Equation~(\ref{tail}) by two. 

We are left with the middle part of Equation~(\ref{total_expectation}) that considers the case of $|x|<\tau$. Note that the qunatizer rounds input values to the nearest discrete value that is a multiple of the quantization step $\Delta$. Hence, the quantization error, $e=x - \Delta\cdot \left\lfloor \frac { x }{ \Delta } \right\rceil$, is uniformly distributed and bounded in the range $[-\frac{\Delta}{2},\frac{\Delta}{2}]$. Hence, we get that 
% \begin{equation}
% \begin{split}
%      \mathbb{E} \left[ \left( x - \Delta\cdot \left\lfloor \frac { x } { \Delta } \right\rceil \right) ^ { 2 } \mid |x|\leq \tau  \right ] &= \int _ { - \frac { \Delta } { 2 } } ^ { \frac { \Delta } { 2 } } \frac { 1 } { \Delta } \cdot e ^ { 2 } de \\
%      &= \frac { \Delta ^ { 2 } } { 12 } \,.
%     \label{MSE}
%     \end{split}
% \end{equation}

\begin{equation}
     \mathbb{E} \left[ \left( x - \Delta\cdot \left\lfloor \frac { x } { \Delta } \right\rceil \right) ^ { 2 } \mid |x|\leq \tau  \right ] = \int _ { - \frac { \Delta } { 2 } } ^ { \frac { \Delta } { 2 } } \frac { 1 } { \Delta } \cdot e ^ { 2 } de \\
     = \frac { \Delta ^ { 2 } } { 12 } \,.
    \label{MSE}
\end{equation}

Finally, we are left to estimate $P \left[ |x| \leq \tau \right]$, which is exactly the probability of sampling a uniform random variable from a range of $2\tau$ out of a total range of $2a$:
\begin{equation}
    P \left[ |x| \leq \tau \right] =  \frac{2\tau}{2a} = \frac{\tau}{a} \,.
\end{equation}

By summing all terms of Equation~(\ref{total_expectation}) and substituting $\tau = 2^{M-1}\Delta$, we achieve the following expression for the expected MSE:
% \begin{equation}
% \label{MSE_uniform}
%     \begin{split} \mathbb{E}\left[\left(x- Q_{\Delta}(x)\right)^2\right]&=
%     {\frac{(a-\tau)^3}{3a} +  \frac{\tau}{a}  \frac { \Delta ^ { 2 } } { 12 } }\\
%     &=\frac{(a-2^{M-1}\Delta)^3}{3a} + \frac{2^M\Delta^3}{24a} \,.  
%     \end{split} 
% \end{equation}
\begin{equation}
\label{MSE_uniform}
    \mathbb{E}\left[\left(x- Q_{\Delta}(x)\right)^2\right]=
    {\frac{(a-\tau)^3}{3a} +  \frac{\tau}{a}  \frac { \Delta ^ { 2 } } { 12 } }\\
    =\frac{(a-2^{M-1}\Delta)^3}{3a} + \frac{2^M\Delta^3}{24a} \,.  
\end{equation}
$\blacksquare$

In \cref{fig:derivatives}(b) we depict the MSE as a function of $\Delta$ value for 4-bit uniform quantization. We show a good agreement between Equation \ref{MSE_uniform} and the synthetic simulations measuring the MSE. 

As defined in \cref{robustness_definition}, we quantify the quantization sensitivity as the increase in MSE in the surrounding of the optimal quantization step $\tilde{\Delta}$. In Lemma~\ref{optimal_clipping} we will find $\tilde{\Delta}$ for a random variable that is uniformly distributed.

\begin{figure}
    \centering
    \begin{subfigure}{0.49\textwidth}
    	\centering
		\includegraphics[height=4.8cm]{imgs/GaussianAnalysis.pdf}
		\caption{\textbf{Optimal quantization of normally distributed tensors.} The first order gradient zeroes at a region with a relatively high-intensity 2nd order gradient, i.e., a region with a high quantization sensitivity $\Gamma(X_N,\varepsilon)$. This sensitivity zeros only asymptotically when $\Delta$ (and MSE) tends to infinity. This means that optimal quantization is highly sensitive to changes in the quantization process.}
		\label{fig:pred_mech:old}
	\end{subfigure}
	~
	\begin{subfigure}{0.49\textwidth}
		\centering
		\includegraphics[height=4.8cm]{imgs/UnifromAnalysis.pdf}
		\caption{\textbf{Optimal quantization of uniformly distributed tensors.} First and second-order gradients zero at a similar point, indicating that the optimum $\tilde{\Delta}$ is attained at a region where quantization sensitivity $\Gamma(X_U,\varepsilon)$  tends to zero. This means that optimal quantization is tolerant and can bear changes in the quantization process without significantly increasing the MSE. \\}
	\end{subfigure}

	\caption{ Quantization needs to be modeled to take into account uncertainty about the precise way it is being done. The best quantization that minimizes the MSE is also the most robust one with uniformly distributed tensors (sub-figure (b)), but not with normally distributed tensors (sub-figure (a)). \textbf{(i) Simulation:}  10,000 values are generated from a uniform/normal distribution and quantized using different quantization step sizes $\Delta$.
	\textbf{(ii) MSE($X,\Delta$):}  Analytical results, stated by Lemma \ref{lemma_uniform_dist} for the uniform case, and developed by \citep{banner2018post} for the normal case - note these are in a
good agreement with simulations. \textbf{(iii) MSE'($X,\Delta$):} The first order derivative zeroes at the region where MSE is minimized. \textbf{(iii) MSE''($X,\Delta$):} second order derivative zeroes in the region with maximum robustness. }
	\label{fig:derivatives}
\end{figure}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\begin{lemma}
\label{optimal_clipping}
Let $X_U$ be a continuous random variable that is uniformly distributed in the interval $[-a,a]$. Given an $M$-bit quantizer $Q_{\Delta}(X)$, the expected MSE $\mathbb{E}\left[\left(X- Q_{\Delta}(X)\right)^2\right]$ is minimized by selecting the following quantization step size:  
\begin{equation}
\tilde{\Delta}= \dfrac{2a}{2^{M}\pm 1} \approx \frac{2a}{2^M} \,.
\end{equation}
\end{lemma}
 
\textbf{Proof:} We calculate the roots of the first order derivative of Equation~(\ref{MSE_uniform}) with respect to $\Delta$ as follows:
% \begin{equation}
% \label{optimal_delta_uniform}
% \begin{split}
%     &\frac{\partial\text{\text{MSE}}(X_U,\Delta)}{\partial \Delta}=\\
%     &\dfrac{1}{a}\left(2^{M-3}\Delta^2-2^{M-1}\left(a-2^{M-1}\Delta\right)^2\right)=0 \,.
% \end{split}
% \end{equation}

\begin{equation}
\label{optimal_delta_uniform}
    \frac{\partial\text{\text{MSE}}(X_U,\Delta)}{\partial \Delta}=\\
    \dfrac{1}{a}\left(2^{M-3}\Delta^2-2^{M-1}\left(a-2^{M-1}\Delta\right)^2\right)=0 \,.
\end{equation}

Solving Equation~(\ref{optimal_delta_uniform}) yields the following solution:
\begin{equation}
  \tilde{\Delta}= \dfrac{2a}{2^{M}\pm 1} \approx \frac{2a}{2^M} \,.
\end{equation}
$\blacksquare$

We can finally provide the main result of this paper, stating that the uniform distribution is more robust to modification in the quantization process compared with the typical distributions of weights and activations that tend to be normal. 
\begin{theorem}
\label{final_theorem}
Let $X_U$ and $X_N$ be continuous random variables with a uniform and normal distributions. Then, for any given $\varepsilon>0$, the quantization sensitivity  $\Gamma(X,\epsilon)$ satisfies the following inequality:
\begin{equation}
    \Gamma(X_U,\epsilon)< \Gamma(X_N,\epsilon) \,,
\label{robustness_equantion}
\end{equation}
i.e., compared to the typical normal distribution, the uniform distribution is more robust to \textbf{changes} in the quantization step size $\Delta$ . 
\end{theorem}
\textbf{Proof:} In the following, we use Lemma \ref{Lemma1} to calculate the quantization sensitivity of each distribution. We begin with the uniform case. We have proven in Lemma \ref{lemma_uniform_dist} the following:
\begin{equation*}
 \text{\text{MSE}}(X_U,\Delta)  = \frac{(a-2^{M-1}\Delta)^3}{3a} + \frac{2^M\cdot\Delta^3}{24a}   \,.
\end{equation*} 
 
 Hence, since we have shown in Lemma \ref{optimal_clipping} that optimal step size for $X_U$ is $\tilde{\Delta}\approx \frac{a}{2^{M-1}}$ we get that 
%  \begin{equation}
%  \begin{split}
%      \Gamma(X_U,\epsilon) &= \left|\frac{\partial^2 \text{mse}(X_U, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \right|\\
%      &=\frac{2^{2M-1}(a-2^{M-1}\tilde{\Delta})+ 2^{M-2}\tilde{\Delta}}{a}\cdot \frac{\epsilon^2}{2} \\
%      &= \frac{\epsilon^2}{4} \,.
%      \end{split}
%  \end{equation}

\begin{equation}
     \Gamma(X_U,\epsilon) = \left|\frac{\partial^2 \text{mse}(X_U, \Delta= \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \right|\\
     =\frac{2^{2M-1}(a-2^{M-1}\tilde{\Delta})+ 2^{M-2}\tilde{\Delta}}{a}\cdot \frac{\epsilon^2}{2} \\
     = \frac{\epsilon^2}{4} \,.
 \end{equation}
 
We now turn to find the sensitivity of the normal distribution $\Gamma(X_N,\epsilon)$. According to \citep{banner2018post}, the expected MSE for the quantization of a Gaussian random variable $N(\mu=0,\sigma)$ is as follows:

% \begin{equation}
% \label{MSE_normal}
% \begin{split}
%  \text{\normalfont{MSE}}(X_N,\Delta) &\approx (\tau^2+\sigma^2)\cdot\left[1-\operatorname{erf}\left(\frac{\tau}{\sqrt{2}\sigma}\right)\right] \\
%  & + \frac{\tau^2}{3\cdot 2^{2M}} - \frac{\sqrt{2}\tau\cdot\sigma\cdot\mathrm{e}^{-\frac{\tau^2}{2\cdot\sigma^2}}}{\sqrt{{\pi}}} \,,
% \end{split}
% \end{equation}

\begin{equation}
\label{MSE_normal}
 \text{\normalfont{MSE}}(X_N,\Delta) \approx (\tau^2+\sigma^2)\cdot\left[1-\operatorname{erf}\left(\frac{\tau}{\sqrt{2}\sigma}\right)\right] \\
  + \frac{\tau^2}{3\cdot 2^{2M}} - \frac{\sqrt{2}\tau\cdot\sigma\cdot\mathrm{e}^{-\frac{\tau^2}{2\cdot\sigma^2}}}{\sqrt{{\pi}}} \,,
\end{equation}

where $\tau= 2^{M-1}\Delta$.

To obtain the quantization sensitivity, we first calculate the second derivative:
% \begin{equation}
% \begin{split}
% &{\frac{\partial^2 \text{MSE}(X_N, \Delta=
% \tilde{\Delta})}{\partial^2 \Delta} =}\\
% &{=\dfrac{2}{3\cdot2^{2M}}-2\operatorname{erf}\left(\dfrac{2^{M-1}\tilde{\Delta}}{\sqrt{2}\sigma}\right)-2} \,.
% \end{split}
% \end{equation}


\begin{equation}
{\frac{\partial^2 \text{MSE}(X_N, \Delta=
\tilde{\Delta})}{\partial^2 \Delta} = }\\
{\dfrac{2}{3\cdot2^{2M}}-2\operatorname{erf}\left(\dfrac{2^{M-1}\tilde{\Delta}}{\sqrt{2}\sigma}\right)-2} \,.
\end{equation}


We have three terms: the first is positive but not larger than $\frac{1}{6}$ (for the case of $M=1$); the second is negative in the range $[-2,0]$; and the third is the constant $-2$. The sum of the three terms falls in the range $[-4,-\frac{11}{6}]$. Hence, the quantization sensitivity for normal distribution is at least 
% \begin{equation}
% \begin{split}
% \Gamma(X_N,\epsilon) =& \\
%       =&\left|\frac{\partial^2 \text{MSE}(X_N, \Delta=
% \tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \right|\geq \frac{11\varepsilon^2}{12} \,.
% \end{split}
% \end{equation}

\begin{equation}
\Gamma(X_N,\epsilon) = \\
      \left|\frac{\partial^2 \text{MSE}(X_N, \Delta=
\tilde{\Delta})}{\partial^2 \Delta} \cdot \frac{\epsilon^2}{2} \right|\geq \frac{11\varepsilon^2}{12} \,.
\end{equation}

This clearly establishes the theorem since we have that  $\Gamma(X_N,\varepsilon)>\Gamma(X_U,\varepsilon)$
$\blacksquare$

\subsection{When robustness and optimality Meet}

We have developed in the previous section the MSE as a function of quantization step size $\Delta$ for the uniform case. We have shown that optimal quantization step size is approximately $\tilde{\Delta}\approx\frac{2a}{2^M}$. The second order derivative is linear in $\Delta$ and zeroes at approximately the same location:
\begin{equation}
    \Delta = \frac{2a}{2^M-\frac{1}{2^M}}\approx \frac{2a}{2^M} \,.
\end{equation}
Therefore, for the uniform case, the optimal quantization step size in terms of  $\text{MSE}(X,\tilde{\Delta})$ is generally the one that optimizes the sensitivity $ \Gamma(X,\epsilon)$, as illustrated by \cref{fig:derivatives}.  


Finally, \cref{fig:mse_for_different_ditribution} presents the minimum MSE distortions for different bit-width when normal and uniform distributions are optimally quantized. These optimal MSE values constitute the optimal solution of equations  \cref{MSE_uniform} and \cref{MSE_normal}, respectively. Note that the optimal quantization of uniformly distributed tensors is superior in terms of MSE to normally distributed tensors at all bit-width representations. 

\begin{figure}[h]
\centering
\includegraphics[height=0.4\textwidth]{imgs/mse_for_different_ditribution.pdf}
\caption{$\text{MSE}(X,\tilde{\Delta})$ as a function of bit-width M for Uniform and Normal distributions. $\text{MSE}(X_U,\tilde{\Delta})$ is significantly smaller than $\text{MSE}(X_N,\tilde{\Delta})$.}
\label{fig:mse_for_different_ditribution}
\end{figure}

In this section, we proved that uniform distribution is more robust to perturbations in quantization parameters than normal distribution.
The robustness of the uniform distribution over Laplace distribution, for example, can be similarly justified.
In the next section, we show how DNN tensor distributions can be manipulated to form different distributions, and in particular to form the uniform distribution.

\section{Kurtosis regularization (\KAT{})}
DNN parameters usually follow Gaussian or Laplace distributions \cite{banner2018post}. However, we would like to obtain the robust qualities that the uniform distribution introduces (\cref{sec:model_problem_formulation}).
\citep{Yu2019GDRQGD} suggested to reshape the model distributions by imposing clipping during training. In this work, we use \emph{kurtosis} --- the fourth standardized moment --- as a proxy to the probability distribution.

\subsection{Kurtosis --- The fourth standardized moment}
The kurtosis of a random variable $\mathcal{X}$ is defined as follows:
\begin{equation}
        \text{Kurt} \left[\mathcal{X}\right] = \mathbb{E} \left[\left( \frac{\mathcal{X} - \mu}{\sigma} \right) ^4 \right]  \,,
    \label{eq:kurt}
\end{equation}
where $\mu$ and $\sigma$ are the mean and standard deviation of $\mathcal{X}$, respectively.
The kurtosis is the fourth central moment normalized by the standard deviation $\sigma$. It provides a scale and shift-invariant measure that captures the shape of the probability distribution $\mathcal{X}$, rather than its mean or variance. If $\mathcal{X}$ is a uniform distributed variable, its kurtosis value will be 1.8, whereas if $\mathcal{X}$ is a normal distributed variable or Laplace distributed variable then its kurtosis values will be 3 and 6, respectively \cite{lawrenceKurt}. We define "kurtosis target", $\mathcal{K}_T$, as the kurtosis value we want the tensor to adopt. In our case, the kurtosis target is 1.8 (uniform distribution). In the following section we describe how we manipulate the model kurtosis.


\subsection{Kurtosis loss}
To control the model weights distributions, we introduce \emph{kurtosis regularization} (\KAT{}).
\KAT{} enables us to control the tensor distribution during training while maintaining the original model accuracy in full precision.

\KAT{} is applied to the model loss function, $\mathcal{L}$, as follows:
\label{method:kurtLoss}
\begin{equation}
        \mathcal{L} = \mathcal{L}_{\text{p}} + \lambda \mathcal{L}_{K} \,,
    \label{eq:losses}
\end{equation}
where $\mathcal{L}_{{p}}$ is the target loss function,
$\mathcal{L}_{K}$ is the \KAT{} term, and $\lambda$ is the \KAT{} coefficient.
$\mathcal{L}_{K}$ is defined as
\begin{equation}
        \mathcal{L}_{K} =  \frac{1}{L}\sum_{i=1}^{L}  \left| \text{Kurt} \left[\mathcal{W}_i\right] - \mathcal{K}_T\right|^2 \,,
    \label{eq:kurtTarget}
\end{equation}
where $L$ is the number of layers and $\mathcal{K}_T$ is the target for kurtosis regularization.

% \begin{figure}[h]
%  \centering
% \includegraphics[width=0.6\linewidth]{imgs/histograms_and_acurracy_for_diff_k_with_axes.png}
%  \caption{The effect of \KAT{} on weight values distribution of one layer in ResNet-18 (top) and ResNet-18 accuracy with PTQ setting (bottom).
%  Uniformization of the model ($\mathcal{K}_T = 1.8$) provides higher accuracy.}
% \label{fig:histograms_and_acc_per_k}
% \end{figure}

\begin{figure}[h]
\centering
\begin{subfigure}{0.45\linewidth}
	\centering
	\includegraphics[height=4.5cm]{imgs/histogram_uniformization_1.pdf}
	\caption{}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
	\centering
	\includegraphics[height=4.7cm]{imgs/kurtosis_val_vs_resnet18_accuracy_for_different_bit_width.pdf}
	\caption{}
\end{subfigure}
 \caption{The effect of \KAT{} on weight values distribution of one layer in ResNet-18 (a) and ResNet-18 accuracy with PTQ setting (b).
 Uniformization of the model ($\mathcal{K}_T = 1.8$) provides higher accuracy.}
\label{fig:histograms_and_acc_per_k}
\end{figure}

To demonstrate the impact of \KAT{}, \cref{fig:histograms_and_acc_per_k} (top) presents weight distributions of one layer from ResNet-18 which was trained with different \KAT{} values.
We also examine the effect of different $\mathcal{K}_T$ values on the accuracy and robustness of an entire ResNet-18 model.
Considering model robustness for different bit-widths, maximum robustness is observed for $\mathcal{K}_T = 1.8$, as expected according to \cref{fig:mse_for_different_ditribution}.
Furthermore, in \cref{fig:quant_sense} we demonstrate the sensitivity of one ResNet-18 layer to the the step size ($\Delta$).
It is clear that a model which was trained with \KAT{} and $\mathcal{K}_T = 1.8$ achieves superior robustness qualities than its non-\KAT{} counterpart (\cref{final_theorem}).

While \KAT{} may be used to achieve different tensor distributions, we use it to achieve uniform-like distributions. We further explore the performance of these models next.

\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth, height=5.0cm]{imgs/QuantSensitivityLsqVs18kurt.pdf}
\caption{Sensitivity of the weights, $\Gamma(X,\varepsilon)$, in one layer of ResNet-18 as a function of the change in the quantization step size from the optimal quantization step size ($\epsilon = |\Delta - \tilde{\Delta}| $). The kurtosis regularization improves the robustness.}
\label{fig:quant_sense}
\end{figure}


==> sections/07_supp_mat_old.tex <==
\section{Hyper parameters to reproduce the results in Section 5- Experiments}

% \MR{write better} Following we described the hyper parameters used in the experiments section. A fully reproducible code accompanies the paper. 

In the following section we describe the hyper parameters used in the experiments section. A fully reproducible code accompanies the paper. 

\subsection{Hyper parameters for Section 5.1- Robustness towards variations in quantization step size}


\subsection{Hyper parameters for Section 5.1 - Post Training Quantization (PTQ) results}
In \cref{ptq_hyper_params_table} we describe the hyper-parameters used in section 5.1.
We apply \KAT{} on a pre-trained model from torch-vision repository and fine-tune it with the following hyper-parameters. All the other hyper-parameters like momentum and w-decay stay the same as in the pre-trained model. 

\begin{table}[h]
\caption{Hyper parameters for experiments in section 5.1 - Post Training Quantization}
\label{ptq_hyper_params_table}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
% \begin{tabular}{| m{1cm} | m{1cm} | m{1cm} | m{1cm} | m{1cm} | m{1cm} | m{1cm} | m{1cm} |}
\begin{tabularx}{\textwidth}{l|m{1.6cm}|m{1.9cm}|m{0.7cm}|m{2cm}|m{0.7cm}|c|m{1.0cm}}
\toprule
architecture & \centering kurtosis target ($\mathcal{K}_T$) & \centering \KAT{} coefficient ($\lambda$ ) & \centering initial lr & \centering lr schedule & \centering batch size & epochs & fp32   accuracy \\
\midrule
ResNet-18    & & & & & \centering 256 & 83 & 70.3 \\
% \midrule{6-8}
\cline{6-8}
\cline{0-0}
ResNet-50    & \multirow{1}{1.6cm}{\centering 1.8} & \multirow{1}{1.9cm}{\centering 1.0} & \multirow{1}{0.7cm}{\centering 0.001} & \multirow{-2}{2.0cm}{\centering decays by a factor of 10 every 30 epochs} & \centering 128 & 49 & 76.4 \\
\cline{6-8}
\cline{0-0}
MobileNet-V2 & & & & & \centering 256 & 83 & 71.3 \\
\bottomrule
\end{tabularx}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\subsection{Hyper parameters for Section 5.2 - Quantization-Aware-Training (QAT) results}
We combine \KAT{} with QAT method during the training phase. In \cref{qat_hyper_params_tables} we describe the hyper-parameters we used.

\begin{table}[h]
\caption{Hyper parameters for experiments in section 5.2 - Quantization Aware Training}
\label{qat_hyper_params_tables}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabularx}{\textwidth}{m{1.2cm}|m{1cm}|m{1.4cm}| m{0.9cm} |m{1.3cm}|m{0.7cm}|m{1.3cm}|m{0.7cm}|m{0.7cm}|m{0.6cm}}
\toprule
\centering arch & \centering QAT method & \centering quantization settings (W/A) & \centering kurtosis target ($\mathcal{K}_T$) & \centering  \KAT{} coefficient ($\lambda$ ) & \centering initial lr & \centering lr schedule & \centering batch size & \centering epochs & acc \\
\midrule
\centering ResNet-18    & \centering DoReFa & \centering 4 / 4 & \centering 1.8 & \centering 1.0 &   1e-4 & \centering decays by a factor of 10 every 30 epochs & \centering 256 & \centering 80 & 68.3 \\
\midrule
\centering ResNet-18    & \centering LSQ & \centering 4 / FP32 & \centering 1.8 & \centering 1.0 & 1e-4 & \centering decays by a factor of 10 every 20 epochs & \centering 128 & \centering 70 & 68.70 \\
\midrule
\centering ResNet-50    & \centering LSQ & \centering 4 / FP32 & \centering 1.8 & \centering 1.0 & 1e-4  & \centering decays by a factor of 10 every 30 epochs & \centering 64 & \centering 18 & 75.7 \\
\midrule
\centering MobileNet-V2 & \centering DoReFa & \centering 4 / FP32 & \centering 1.8 & \centering 1.0 & \centering 5e-5 & \centering lr decay rate of 0.98 per epoch & \centering 128 & \centering 10 & 66.9 \\
\bottomrule
\end{tabularx}
\end{small}
\end{center}
\vskip -0.1in
\end{table}




\section{Mean and standard deviation over multiple runs of ResNet-18 trained with DoReFa and KURE}

\begin{table}[h!]
\caption{Mean and standard deviation over multiple runs of ResNet-18 trained with DoReFa and KURE}
\label{mean_std_resnet18_dorefa}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{tabular}{\textwidth}{l|m{1cm}|m{1.6cm}|c|m{2cm}}
\begin{tabular}{l|m{1cm}|m{1.6cm}|c|m{2cm}}
\toprule
architecture & \centering QAT method & \centering quantization settings (W/A) & Runs & Accuracy, \% ($mean \pm std$) \\
\midrule
ResNet-18 & DoReFa & \centering 4 / 4 & 3 & ($68.4 \pm 0.09 $) \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\begin{figure}[h!]
 \centering
\includegraphics[width=0.45\linewidth, height=5.5cm]{imgs/qat_dorefa_sensitivity_resnet18_accu_for_different_scale_ratio_mult_runs.pdf}
\caption{The network has been trained for quantization step size $\Delta^*$. Still, the quantizer uses a slightly different step size $\Delta$. Small changes in optimal step size $\Delta^*$ cause severe accuracy degradation in the quantized model. \KAT{} significantly enhances the model robustness by promoting solutions that are more robust to uncertainties in the quantizer design (ResNet-18 on ImageNet).}
\label{fig:scaleRatop_mean_std}
\end{figure}

